New results on the spectroscopy of XYZ states from LHC experiments

The main results from LHC experiments on XYZ charmonium-like candidates are summarized.

==> my-def.tex <==
\newcommand \TwoColumns[4]{
\begin{columns}[C]
   \begin{column}{#1}
   #2
   \end{column}
   \begin{column}{#3}
   #4
   \end{column}
\end{columns}}

\newcommand \ThreeColumns[6]{
\begin{columns}[C]
   \begin{column}{#1}
   #2
   \end{column}
   \begin{column}{#3}
   #4
   \end{column}
   \begin{column}{#5}
   #6
   \end{column}
\end{columns}}
